Self-Supervised GAN to Counter Forgetting

GANs involve training two networks in an adversarial game, where each network's task depends on its adversary. Recently, several works have framed GAN training as an online or continual learning problem. We focus on the discriminator, which must perform classification under an (adversarially) shifting data distribution. When trained on sequential tasks, neural networks exhibit \emph{forgetting}. For GANs, discriminator forgetting leads to training instability. To counter forgetting, we encourage the discriminator to maintain useful representations by adding a self-supervision. Conditional GANs have a similar effect using labels. However, our self-supervised GAN does not require labels, and closes the performance gap between conditional and unconditional models. We show that, in doing so, the self-supervised discriminator learns better representations than regular GANs.

==> content/conclusion.tex <==
\section{Conclusion}
Based on the intuition discriminator can have a hard time learning representation in non-stationary setting, we proposed to adopt self-supervised method to enhance GAN training, which closes the performance gap between conditional and unconditional GANs.

%In this work, we analyze the importance of representation learning for discriminators in generative adversarial networks, and found that in order for the generator to generate meaningful real data (e.g. images), the discriminator needs to learn the representations. Based on the observation, we propose a self-supervised enhance discriminator for GANs. The proposed method is simple yet effective, closing the performance gaps between unconditional and conditional generative models.
